Unsupervised cycle-consistent deformation for shape matching

We propose a self-supervised approach to deep surface deformation. Given a pair of shapes, our algorithm directly predicts a parametric transformation from one shape to the other respecting correspondences. Our insight is to use cycle-consistency to define a notion of good correspondences in groups of objects and use it as a supervisory signal to train our network. Our method does not rely on a template, assume near isometric deformations or rely on point-correspondence supervision. We demonstrate the efficacy of our approach by using it to transfer segmentation across shapes. We show, on Shapenet, that our approach is competitive with comparable state-of-the-art methods when annotated training data is readily available, but outperforms them by a large margin in the few-shot segmentation scenario.

==> qualitative_results.tex <==
\begin{figure*}[!t!]
\vspace{-1.0cm}
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}{0.145\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success1_testSample_bw.png} \\
\vspace{-1.8cm}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success2_testSample_bw.png} \\
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success1_testSample_bw.png} \\
\vspace{-1.6cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success2_testSample_bw.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success1_testSample_bw.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success2_testSample_bw.png} \\
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success1_testSample_bw.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success2_testSample_bw.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success1_testSample_bw.png} \\
\vspace{-0.5cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success2_testSample_bw.png} \\
\vspace{-0.7cm}
%
\caption{Input shape \\ (target)}
\end{subfigure}
\begin{subfigure}{0.145\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success1_trainSample.png} \\
\vspace{-1.8cm}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success2_trainSample.png} \\
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success1_trainSample.png} \\
\vspace{-1.6cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success2_trainSample.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success1_trainSample.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success2_trainSample.png} \\
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success1_trainSample.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success2_trainSample.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success1_trainSample.png} \\
\vspace{-0.5cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success2_trainSample.png} \\
\vspace{-0.7cm}
%
\caption{Retrieved shape \\ (source)}
\end{subfigure}
\begin{subfigure}{0.145\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success1_trainDeformed.png} \\
\vspace{-1.8cm}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success2_trainDeformed.png} \\
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success1_trainDeformed.png} \\
\vspace{-1.6cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success2_trainDeformed.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success1_trainDeformed.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success2_trainDeformed.png} \\
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success1_trainDeformed.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success2_trainDeformed.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success1_trainDeformed.png} \\
\vspace{-0.5cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success2_trainDeformed.png} \\
\vspace{-0.7cm}
%
\caption{Deformed \\ retrieved shape}
\end{subfigure}
\begin{subfigure}{0.145\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success1_testOur.png} \\
\vspace{-1.8cm}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success2_testOur.png} \\
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success1_testOur.png} \\
\vspace{-1.6cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success2_testOur.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success1_testOur.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success2_testOur.png} \\
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success1_testOur.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success2_testOur.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success1_testOur.png} \\
\vspace{-0.5cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success2_testOur.png} \\
\vspace{-0.7cm}
%
\caption{Transferred labels \\ to input}
\end{subfigure}
\begin{subfigure}{0.145\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success1_testSample.png} \\
\vspace{-1.8cm}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success2_testSample.png} \\
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success1_testSample.png} \\
\vspace{-1.6cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success2_testSample.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success1_testSample.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success2_testSample.png} \\
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success1_testSample.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success2_testSample.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success1_testSample.png} \\
\vspace{-0.5cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success2_testSample.png} \\
\vspace{-0.7cm}
\caption{Ground truth \\ labels}
\end{subfigure}
\begin{subfigure}{0.145\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success1_testNN.png} \\
\vspace{-1.8cm}
\includegraphics[width=\linewidth]{figures/success/Airplane/best_Success2_testNN.png} \\
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success1_testNN.png} \\
\vspace{-1.6cm}
\includegraphics[width=\linewidth]{figures/success/Car/best_Success2_testNN.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success1_testNN.png} \\
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/best_Success2_testNN.png} \\
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success1_testNN.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/best_Success2_testNN.png} \\
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success1_testNN.png} \\
\vspace{-0.5cm}
\includegraphics[width=\linewidth]{figures/success/Table/best_Success2_testNN.png} \\
\vspace{-0.7cm}
%
\caption{Identity baseline \\ segmentation}
\end{subfigure}
\caption{\textbf{Qualitative results.} 
For each input shape (a), we select the top nearest neighbor from 400 training examples with part segmentations using the cycle-consistency criterion (b). We apply our approach to deform the retrieved shape to align with the input shape (c). Given the deformed shape, we transfer the labels onto the input shape (d). For each category, we show the top results that maximize IoU with the ground truth (e). For comparison, we show the Identity baseline in (f). Notice how our method successfully transfers labels and improves over the baseline.
%
}
 \label{fig:bestresultsoveridentity}
 \vspace*{-4mm}
\end{figure*}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\begin{figure*}[!t!]
\centering
\captionsetup[subfigure]{justification=centering}
\begin{subfigure}{0.15\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/worse_Failure1_testSample_bw.png} \\
%
%
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/worse_Failure1_testSample_bw.png} \\
%
%
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/worse_Failure1_testSample_bw.png} \\
%
%
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/worse_Failure1_testSample_bw.png} \\
%
%
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/worse_Failure1_testSample_bw.png} \\
%
%
\vspace{-0.7cm}
%
\caption{Input shape \\ (target)}
\end{subfigure}
\begin{subfigure}{0.15\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/worse_Failure1_trainSample.png} \\
%
%
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/worse_Failure1_trainSample.png} \\
%
%
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/worse_Failure1_trainSample.png} \\
%
%
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/worse_Failure1_trainSample.png} \\
%
%
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/worse_Failure1_trainSample.png} \\
%
%
\vspace{-0.7cm}
%
\caption{Retrieved shape \\ (source)}
\end{subfigure}
\begin{subfigure}{0.15\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/worse_Failure1_trainDeformed.png} \\
%
%
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/worse_Failure1_trainDeformed.png} \\
%
%
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/worse_Failure1_trainDeformed.png} \\
%
%
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/worse_Failure1_trainDeformed.png} \\
%
%
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/worse_Failure1_trainDeformed.png} \\
%
%
\vspace{-0.7cm}
%
\caption{Deformed \\ retrieved shape}
\end{subfigure}
\begin{subfigure}{0.15\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/worse_Failure1_testOur.png} \\
%
%
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/worse_Failure1_testOur.png} \\
%
%
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/worse_Failure1_testOur.png} \\
%
%
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/worse_Failure1_testOur.png} \\
%
%
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/worse_Failure1_testOur.png} \\
%
%
\vspace{-0.7cm}
%
\caption{Transferred labels \\ to input}
\end{subfigure}
\begin{subfigure}{0.15\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/worse_Failure1_testSample.png} \\
%
%
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/worse_Failure1_testSample.png} \\
%
%
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/worse_Failure1_testSample.png} \\
%
%
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/worse_Failure1_testSample.png} \\
%
%
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/worse_Failure1_testSample.png} \\
%
%
\vspace{-0.7cm}
%
\caption{Ground truth \\ labels}
\end{subfigure}
\begin{subfigure}{0.15\linewidth}
\includegraphics[width=\linewidth]{figures/success/Airplane/worse_Failure1_testNN.png} \\
%
%
\vspace{-1.2cm}
\includegraphics[width=\linewidth]{figures/success/Car/worse_Failure1_testNN.png} \\
%
%
\vspace{-1.0cm}
\includegraphics[width=\linewidth]{figures/success/Chair/worse_Failure1_testNN.png} \\
%
%
\vspace{-0.4cm}
\includegraphics[width=\linewidth]{figures/success/Lamp/worse_Failure1_testNN.png} \\
%
%
\vspace{-0.8cm}
\includegraphics[width=\linewidth]{figures/success/Table/worse_Failure1_testNN.png} \\
%
%
\vspace{-0.7cm}
%
\caption{Identity baseline \\ segmentation}
\end{subfigure}
\caption{\textbf{Failures.} 
Example failures include when a retrieved shape has inconsistent annotation (rows 1,2,5) and poor deformation due to different topology (rows 3,4).
%
}
 \label{fig:failurecases}
 \vspace*{-4mm}
\end{figure*}


